PAC Prediction Sets for Meta-Learning

Uncertainty quantification is a key component of machine learning models targeted at safety-critical systems such as in healthcare or autonomous vehicles. We study this problem in the context of meta learning, where the goal is to quickly adapt a predictor to new tasks. In particular, we propose a novel algorithm to construct \emph{PAC prediction sets}, which capture uncertainty via sets of labels, that can be adapted to new tasks with only a few training examples. These prediction sets satisfy an extension of the typical PAC guarantee to the meta learning setting; in particular, the PAC guarantee holds with high probability over future tasks. We demonstrate the efficacy of our approach on four datasets across three application domains: mini-ImageNet and CIFAR10-C in the visual domain, FewRel in the language domain, and the CDC Heart Dataset in the medical domain. In particular, our prediction sets satisfy the PAC guarantee while having smaller size compared to other baselines that also satisfy this guarantee.

==> sections/method_bu.tex <==
%% !TEX root = ../main.tex
\section{Meta PAC Prediction Sets}
We propose a PAC prediction set for meta learning.
In particular, we consider a meta-learned score function, 
which is typically trained to be a good predictor after adaptation to the test distribution.
Our prediction set has a correctness guarantee for future test distributions. 

{\color{red}
%We describe a high-level overview on prediction set construction in a meta learning setup and our approach.
%% problem
There are three sources of randomness: (1) an adaptation set and a calibration set for each calibration task, (2) an adaptation set for a new task, and (3) an evaluation set for the same new task. 
We control the three sources of randomness and error by $\delta$, $\alpha$, and $\ep$, respectively, aiming to construct a prediction set that contains labels from a new task. 
%% approach: an interval over parameters
Given a meta-learned model, the proposed algorithm consists of two steps: 
constructing a prediction set---captured by a specific parameter to be specified below---for each calibration task (related to $\ep$ and $\alpha$), and 
then
constructing a prediction interval over parameters (related to $\alpha$ and $\delta$).

% an interval over thresholds
Suppose we have prediction sets for each task, parametrized by some threshold parameters.
Suppose that,  for each task, the parameters only depend on an adaptation set for the respective task. As tasks are i.i.d., the parameters also turn out to be i.i.d.. 
The distribution of parameters represents a possible range of the parameter for a new task. 
In particular, if for each task,  the prediction set contains the true label a fraction $1 - \epsilon$ of the time, the distribution of the parameters 
suggests how one may achieve
$\epsilon$-correct prediction sets for a new task. 
Based on this observation, we construct a prediction interval that contains a fraction $1 - \alpha$  of  $\epsilon$-correct prediction set parameters. 
% randomness from calibration tasks
However, the parameters of prediction sets need to be estimated from calibration tasks, and the estimated parameters depend on the randomness of calibration tasks. 
Thus, we construct a prediction interval over parameters which accounts for this randomness. 
The interval is chosen to be correct 
(\ie to contains $\epsilon$-correct prediction set parameters for a fraction $1 - \alpha$ of new tasks) with probability at least $1 - \delta$ over the randomness of calibration tasks.

}


\subsection{Setup and Problem}\label{sec:prob}



\begin{figure}[t]
    \centering
    \small
    \newcommand\SCALE{0.62}
    \newcommand\R{1.0cm}
    \newcommand\RFIX{0.5cm}
    \newcommand\ROWSP{0.3cm}
    \newcommand\COLSP{0.3cm}
    
    \begin{subfigure}[b]{0.44\linewidth}
      \centering
      \scalebox{\SCALE}{
      \begin{tikzpicture}
      
        % theta
        \node [
            circle,
            minimum width=\RFIX,
            minimum height=\RFIX,
        ] (theta) at (0, 0) {
	  \makecell{
            $\theta$
          }
        };
        
        % x
        \node [
            circle,
            draw,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            below=\ROWSP of theta
        ] (x) {
	  \makecell{
            $x$
          }
        };
        % S
        \node [
            circle,
            draw,
            %fill=gray!20,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            left=\COLSP of x
        ] (S) {
	  \makecell{
            $S$
          }
        };
        % y
        \node [
            circle,
            draw,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            right=\COLSP of x
        ] (y) {
	  \makecell{
            $y$
          }
        };
        
%         % tau
%         \node [
%             circle,
%             draw,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of S
%         ] (tau) {
% 	  \makecell{
%             $\tau$
%           }
%         };
        
        % error
        \node [
            rectangle,
            rounded corners,
            draw,
            minimum width=\R*2,
            minimum height=\R,
            below=\ROWSP of $(x.south)!.5!(y.south)$
        ] (error) {
	  \makecell{
            $\mathbbm{1}(y \notin F'(x; S))$
          }
        };
        
        % connectors
        \draw[-stealth] (theta) -- node[midway,left] {} (S);
        \draw[-stealth] (theta) -- node[midway,left] {} (x);
        \draw[-stealth] (theta) -- node[midway,left] {} (y);
        \draw[-stealth] (S) -- node[midway,left] {} (error);
        \draw[-stealth] (x) -- node[midway,left] {} (error);
        \draw[-stealth] (y) -- node[midway,left] {} (error);
        %\draw[-stealth] (tau) -- node[midway,left] {} (error);

      \end{tikzpicture}
      }
      \caption{Marginal guarantee \citep{vovk2005algorithmic}}
      \label{fig:graph:a}
    \end{subfigure}
    \begin{subfigure}[b]{0.44\linewidth}
      \centering
      \scalebox{\SCALE}{
      \begin{tikzpicture}
      
        % theta
        \node [
            circle,
            minimum width=\RFIX,
            minimum height=\RFIX,
        ] (theta) at (0, 0) {
	  \makecell{
            $\theta$
          }
        };
        
        % x
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            minimum width=\R,
            minimum height=\R,
            below=\ROWSP of theta
        ] (x) {
	  \makecell{
            $x$
          }
        };
        % S
        \node [
            circle,
            draw,
            %fill=gray!20,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            left=\COLSP of x
        ] (S) {
	  \makecell{
            $S$
          }
        };
        % y
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            minimum width=\R,
            minimum height=\R,
            right=\COLSP of x
        ] (y) {
	  \makecell{
            $y$
          }
        };
        
        % tau
        \node [
            circle,
            draw,
            minimum width=\R,
            minimum height=\R,
            below=\ROWSP of S
        ] (tau) {
	  \makecell{
            $\tau$
          }
        };
        
        % error
        \node [
            rectangle,
            rounded corners,
            draw,
            minimum width=\R*2,
            minimum height=\R,
            below=\ROWSP of $(x.south)!.5!(y.south)$
        ] (error) {
	  \makecell{
            $\mathbbm{1}(y \notin F_\tau(x))$
          }
        };
        
        % connectors
        \draw[-stealth] (theta) -- node[midway,left] {} (S);
        \draw[-stealth] (theta) -- node[midway,left] {} (x);
        \draw[-stealth] (theta) -- node[midway,left] {} (y);
        \draw[-stealth] (S) -- node[midway,left] {} (tau);
        \draw[-stealth] (x) -- node[midway,left] {} (error);
        \draw[-stealth] (y) -- node[midway,left] {} (error);
        \draw[-stealth] (tau) -- node[midway,left] {} (error);

      \end{tikzpicture}
      }
      \caption{PAC guarantee \citep{wilks1941determination,vovk2013conditional,Park2020PAC}
      \footnotemark
      }
      \label{fig:graph:b}
    \end{subfigure}
    
%     \begin{subfigure}[b]{0.44\linewidth}
%       \centering
%       \scalebox{\SCALE}{
%         \begin{tikzpicture}
%         % theta
%         \node [
%             circle,
%             draw,
%             %pattern=north west lines,
%             %pattern color=gray!40,
%             pattern=north east lines,
%             pattern color=blue!40,
%             minimum width=\R,
%             minimum height=\R,
%         ] (theta) at (0, 0) {
% 	  \makecell{
%             $\theta$
%           }
%         };
        
%         % x
%         \node [
%             circle,
%             draw,
%             pattern=north east lines,
%             pattern color=blue!40,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of theta
%         ] (x) {
% 	  \makecell{
%             $x$
%           }
%         };
% %         % A
% %         \node [
% %             circle,
% %             draw,
% %             %fill=gray!20,
% %             minimum width=\R,
% %             minimum height=\R,
% %             left=\COLSP of x
% %         ] (S) {
% % 	  \makecell{
% %             $A$
% %           }
% %         };
%         % y
%         \node [
%             circle,
%             draw,
%             pattern=north east lines,
%             pattern color=blue!40,
%             minimum width=\R,
%             minimum height=\R,
%             right=\COLSP of x
%         ] (y) {
% 	  \makecell{
%             $y$
%           }
%         };
        
%         % error
%         \node [
%             rectangle,
%             rounded corners,
%             draw,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of $(x.south)!.5!(y.south)$
%         ] (error) {
% 	      \makecell{
%             $\mathbbm{1}(y \notin F'(x; S_{1:N})$
%           }
%         };
        
%         % metaS
%         \node [
%             circle,
%             draw,
%             pattern=north west lines,
%             pattern color=red!40,
%             minimum width=\R,
%             minimum height=\R,
%             left=\ROWSP of x
%         ] (metaS) {
% 	        \makecell{
%                 $S_i$
%             }
%         };
        
%         % % metaA
%         % \node [
%         %     circle,
%         %     draw,
%         %     fill=gray!20,
%         %     minimum width=\R,
%         %     minimum height=\R,
%         %     left=\ROWSP of metaS
%         % ] (metaA) {
% 	       % \makecell{
%         %         $A_i$
%         %     }
%         % };
        
%         % metatheta
%         \node [
%             circle,
%             draw,
%             pattern=north west lines,
%             pattern color=red!40,
%             minimum width=\R,
%             minimum height=\R,
%             above=\ROWSP of metaS
%         ] (metatheta) {
% 	        \makecell{
%                 $\theta_i$
%             }
%         };
        
%         % % metatau
%         % \node [
%         %     circle,
%         %     draw,
%         %     minimum width=\R,
%         %     minimum height=\R,
%         %     below=\ROWSP of metaS
%         % ] (metatau) {
% 	       % \makecell{
%         %         $\tau$
%         %     }
%         % };
        
        
%         % alpha
%         \node [
%             circle,
%             minimum width=\RFIX,
%             minimum height=\RFIX,
%             above=\ROWSP of $(metatheta.north)!.5!(theta.north)$
%         ] (alpha)  {
% 	  \makecell{
%             $\pi$
%           }
%         };
        
%         % N
%         \node [
%             %circle,
%             %minimum width=0.01,
%             %minimum height=0.01,
%             left=0.1 of metatheta
%         ] (K)  {
% 	    \makecell{
%             $N$
%           }
%         };
        
%          % plate
%         \node [
%           draw=black,
%           rounded corners,
%           %dashed,
%           %thick,
%           fit={(metatheta) (metaS) (K)},
%           label={}
%         ] {};
        
%         % connectors
%         %\draw[-stealth] (theta) -- node[midway,left] {} (S);
%         \draw[-stealth] (theta) -- node[midway,left] {} (x);
%         \draw[-stealth] (theta) -- node[midway,left] {} (y);
%         %\draw[-stealth] (S) -- node[midway,left] {} (error);
%         \draw[-stealth] (x) -- node[midway,left] {} (error);
%         \draw[-stealth] (y) -- node[midway,left] {} (error);
%         %\draw[-stealth] (f) -- node[midway,left] {} (error);
%         \draw[-stealth] (alpha) -- node[midway,left] {} (metatheta);
%         \draw[-stealth] (alpha) -- node[midway,left] {} (theta);
%         \draw[-stealth] (metatheta) -- node[midway,left] {} (metaS);
%         %\draw[-stealth] (metatau) -- node[midway,left] {} (error);
%         %\draw[-stealth] (metatheta) -- node[midway,left] {} (metaA);
%         %\draw[-stealth] (metaA) -- node[midway,left] {} (metatau);
%         \draw[-stealth] (metaS) -- node[midway,left] {} (error);
        

%       \end{tikzpicture}
%       }
%       \caption{Meta task-marginal guarantee w/o adaptation}
%       \label{fig:graph:c}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.44\linewidth}
%       \centering
%       \scalebox{\SCALE}{
%       \begin{tikzpicture}
      
        
%         % theta
%         \node [
%             circle,
%             draw,
%             pattern=north east lines,
%             pattern color=blue!40,
%             minimum width=\R,
%             minimum height=\R,
%         ] (theta) at (0, 0) {
% 	  \makecell{
%             $\theta$
%           }
%         };
        
%         % x
%         \node [
%             circle,
%             draw,
%             pattern=horizontal lines,
%             pattern color=ForestGreen!40,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of theta
%         ] (x) {
% 	  \makecell{
%             $x$
%           }
%         };
% %         % A
% %         \node [
% %             circle,
% %             draw,
% %             fill=gray!20,
% %             minimum width=\R,
% %             minimum height=\R,
% %             left=\COLSP of x
% %         ] (S) {
% % 	  \makecell{
% %             $A$
% %           }
% %         };
%         % y
%         \node [
%             circle,
%             draw,
%             pattern=horizontal lines,
%             pattern color=ForestGreen!40,
%             minimum width=\R,
%             minimum height=\R,
%             right=\COLSP of x
%         ] (y) {
% 	  \makecell{
%             $y$
%           }
%         };
        
% %         % f
% %         \node [
% %             circle,
% %             draw,
% %             fill=gray!20,
% %             minimum width=\R,
% %             minimum height=\R,
% %             below=\ROWSP of S
% %         ] (f) {
% % 	  \makecell{
% %             $f$
% %           }
% %         };
        
%         % error
%         \node [
%             rectangle,
%             rounded corners,
%             draw,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of $(x.south)!.5!(y.south)$
%         ] (error) {
% 	      \makecell{
%             $\mathbbm{1}( y \notin F_\tau(x))$
%           }
%         };
        
%         % metaS
%         \node [
%             circle,
%             draw,
%             pattern=north west lines,
%             pattern color=red!40,
%             minimum width=\R,
%             minimum height=\R,
%             left=\ROWSP of x
%         ] (metaS) {
% 	        \makecell{
%                 $S_i$
%             }
%         };
        
%         % % metaA
%         % \node [
%         %     circle,
%         %     draw,
%         %     fill=gray!20,
%         %     minimum width=\R,
%         %     minimum height=\R,
%         %     left=\ROWSP of metaS
%         % ] (metaA) {
% 	       % \makecell{
%         %         $A_i$
%         %     }
%         % };
        
%         % metatheta
%         \node [
%             circle,
%             draw,
%             pattern=north west lines,
%             pattern color=red!40,
%             minimum width=\R,
%             minimum height=\R,
%             above=\ROWSP of metaS
%         ] (metatheta) {
% 	        \makecell{
%                 $\theta_i$
%             }
%         };
        
%         % metatau
%         \node [
%             circle,
%             draw,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of metaS
%         ] (metatau) {
% 	        \makecell{
%                 $\tau$
%             }
%         };
        
        
%         % alpha
%         \node [
%             circle,
%             minimum width=\RFIX,
%             minimum height=\RFIX,
%             above=\ROWSP of $(metatheta.north)!.5!(theta.north)$
%         ] (alpha)  {
% 	  \makecell{
%             $\pi$
%           }
%         };
        
%         % N
%         \node [
%             %circle,
%             %minimum width=0.01,
%             %minimum height=0.01,
%             left=0.1 of metatheta
%         ] (K)  {
% 	    \makecell{
%             $N$
%           }
%         };
        
%          % plate
%         \node [
%           draw=black,
%           rounded corners,
%           %dashed,
%           %thick,
%           fit={(metatheta) (metaS) (K)},
%           label={}
%         ] {};
        
%         % connectors
%         %\draw[-stealth] (theta) -- node[midway,left] {} (S);
%         \draw[-stealth] (theta) -- node[midway,left] {} (x);
%         \draw[-stealth] (theta) -- node[midway,left] {} (y);
%         %\draw[-stealth] (S) -- node[midway,left] {} (error);
%         \draw[-stealth] (x) -- node[midway,left] {} (error);
%         \draw[-stealth] (y) -- node[midway,left] {} (error);
%         \draw[-stealth] (alpha) -- node[midway,left] {} (metatheta);
%         \draw[-stealth] (alpha) -- node[midway,left] {} (theta);
%         \draw[-stealth] (metatheta) -- node[midway,left] {} (metaS);
%         \draw[-stealth] (metatau) -- node[midway,left] {} (error);
%         %\draw[-stealth] (metatheta) -- node[midway,left] {} (metaA);
%         %\draw[-stealth] (metaA) -- node[midway,left] {} (metatau);
%         \draw[-stealth] (metaS) -- node[midway,left] {} (metatau);
        

%       \end{tikzpicture}
%       }
%       \caption{Meta PAC guarantee w/o adaptation (ours)}
%       \label{fig:graph:d}
%     \end{subfigure}
    
    
    \begin{subfigure}[b]{0.44\linewidth}
      \centering
      \scalebox{\SCALE}{
        \begin{tikzpicture}
        % theta
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            %pattern=north west lines,
            %pattern color=gray!40,
            minimum width=\R,
            minimum height=\R,
        ] (theta) at (0, 0) {
	  \makecell{
            $\theta$
          }
        };
        
        % x
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            minimum width=\R,
            minimum height=\R,
            below=\ROWSP of theta
        ] (x) {
	  \makecell{
            $x$
          }
        };
        % A
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            %fill=gray!20,
            minimum width=\R,
            minimum height=\R,
            left=\COLSP of x
        ] (S) {
	  \makecell{
            $A$
          }
        };
        % y
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            minimum width=\R,
            minimum height=\R,
            right=\COLSP of x
        ] (y) {
	  \makecell{
            $y$
          }
        };
        
        % error
        \node [
            rectangle,
            rounded corners,
            draw,
            minimum width=\R*2,
            minimum height=\R,
            %below=\ROWSP of $(x.south)!.5!(y.south)$
            below=\ROWSP of x
        ] (error) {
	      \makecell{
            $\mathbbm{1}(y \notin F'(A, x; A_{1:N}, S_{1:N})$
          }
        };
        
        % metaS
        \node [
            circle,
            draw,
            pattern=north west lines,
            pattern color=red!40,
            %fill=gray!20,
            minimum width=\R,
            minimum height=\R,
            left=\ROWSP of S
        ] (metaS) {
	        \makecell{
                $S_i$
            }
        };
        
        % metaA
        \node [
            circle,
            draw,
            pattern=north west lines,
            pattern color=red!40,
            %fill=gray!20,
            minimum width=\R,
            minimum height=\R,
            left=\ROWSP of metaS
        ] (metaA) {
	        \makecell{
                $A_i$
            }
        };
        
        % metatheta
        \node [
            circle,
            draw,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            above=\ROWSP of metaS
        ] (metatheta) {
	        \makecell{
                $\theta_i$
            }
        };
        
        % % metatau
        % \node [
        %     circle,
        %     draw,
        %     minimum width=\R,
        %     minimum height=\R,
        %     below=\ROWSP of metaS
        % ] (metatau) {
	       % \makecell{
        %         $\tau$
        %     }
        % };
        
        
        % alpha
        \node [
            circle,
            minimum width=\RFIX,
            minimum height=\RFIX,
            above=\ROWSP of $(metatheta.north)!.5!(theta.north)$
        ] (alpha)  {
	  \makecell{
            $\pi$
          }
        };
        
        % N
        \node [
            %circle,
            %minimum width=0.01,
            %minimum height=0.01,
            left=0.6 of metatheta
        ] (K)  {
	    \makecell{
            $N$
          }
        };
        
         % plate
        \node [
          draw=black,
          rounded corners,
          %dashed,
          %thick,
          fit={(metatheta) (metaS) (K) (metaA)},
          label={}
        ] {};
        
        % connectors
        \draw[-stealth] (theta) -- node[midway,left] {} (S);
        \draw[-stealth] (theta) -- node[midway,left] {} (x);
        \draw[-stealth] (theta) -- node[midway,left] {} (y);
        \draw[-stealth] (S) -- node[midway,left] {} (error);
        \draw[-stealth] (x) -- node[midway,left] {} (error);
        \draw[-stealth] (y) -- node[midway,left] {} (error);
        %\draw[-stealth] (f) -- node[midway,left] {} (error);
        \draw[-stealth] (alpha) -- node[midway,left] {} (metatheta);
        \draw[-stealth] (alpha) -- node[midway,left] {} (theta);
        \draw[-stealth] (metatheta) -- node[midway,left] {} (metaS);
        %\draw[-stealth] (metatau) -- node[midway,left] {} (error);
        \draw[-stealth] (metatheta) -- node[midway,left] {} (metaA);
        \draw[-stealth] (metaA) to [bend right=20] node[midway,left] {} (error);
        \draw[-stealth] (metaS) to [bend right=10] node[midway,left] {} (error);
        

      \end{tikzpicture}
      }
      \caption{Meta task-marginal guarantee \citep{fisch2021fewshot}}
      \label{fig:graph:meta-cp}
    \end{subfigure}
    \begin{subfigure}[b]{0.44\linewidth}
      \centering
      \scalebox{\SCALE}{
      \begin{tikzpicture}
      
        
        % theta
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            minimum width=\R,
            minimum height=\R,
        ] (theta) at (0, 0) {
	  \makecell{
            $\theta$
          }
        };
        
        % x
        \node [
            circle,
            draw,
            pattern=horizontal lines,
            pattern color=ForestGreen!40,
            minimum width=\R,
            minimum height=\R,
            below=\ROWSP of theta
        ] (x) {
	  \makecell{
            $x$
          }
        };
        % A
        \node [
            circle,
            draw,
            pattern=north east lines,
            pattern color=blue!40,
            %fill=gray!20,
            minimum width=\R,
            minimum height=\R,
            left=\COLSP of x
        ] (S) {
	  \makecell{
            $A$
          }
        };
        % y
        \node [
            circle,
            draw,
            pattern=horizontal lines,
            pattern color=ForestGreen!40,
            minimum width=\R,
            minimum height=\R,
            right=\COLSP of x
        ] (y) {
	  \makecell{
            $y$
          }
        };
        
%         % f
%         \node [
%             circle,
%             draw,
%             fill=gray!20,
%             minimum width=\R,
%             minimum height=\R,
%             below=\ROWSP of S
%         ] (f) {
% 	  \makecell{
%             $f$
%           }
%         };
        
        % error
        \node [
            rectangle,
            rounded corners,
            draw,
            minimum width=\R*2,
            minimum height=\R,
            %below=\ROWSP of $(x.south)!.5!(y.south)$
            below=\ROWSP of x
        ] (error) {
	      \makecell{
            $\mathbbm{1}( y \notin F_\tau(A, x) )$
          }
        };
        
        % metaS
        \node [
            circle,
            draw,
            %fill=gray!20,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            left=\ROWSP of S
        ] (metaS) {
	        \makecell{
                $S_i$
            }
        };
        
        % metaA
        \node [
            circle,
            draw,
            %fill=gray!20,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            left=\ROWSP of metaS
        ] (metaA) {
	        \makecell{
                $A_i$
            }
        };
        
        % metatheta
        \node [
            circle,
            draw,
            pattern=north west lines,
            pattern color=red!40,
            minimum width=\R,
            minimum height=\R,
            above=\ROWSP of metaS
        ] (metatheta) {
	        \makecell{
                $\theta_i$
            }
        };
        
        % metatau
        \node [
            circle,
            draw,
            minimum width=\R,
            minimum height=\R,
            below=\ROWSP of metaS
        ] (metatau) {
	        \makecell{
                $\tau$
            }
        };
        
        
        % alpha
        \node [
            circle,
            minimum width=\RFIX,
            minimum height=\RFIX,
            above=\ROWSP of $(metatheta.north)!.5!(theta.north)$
        ] (alpha)  {
	  \makecell{
            $\pi$
          }
        };
        
        % N
        \node [
            %circle,
            %minimum width=0.01,
            %minimum height=0.01,
            left=0.6 of metatheta
        ] (K)  {
	    \makecell{
            $N$
          }
        };
        
         % plate
        \node [
          draw=black,
          rounded corners,
          %dashed,
          %thick,
          fit={(metatheta) (metaS) (K) (metaA)},
          label={}
        ] {};
        
        % connectors
        \draw[-stealth] (theta) -- node[midway,left] {} (S);
        \draw[-stealth] (theta) -- node[midway,left] {} (x);
        \draw[-stealth] (theta) -- node[midway,left] {} (y);
        \draw[-stealth] (S) -- node[midway,left] {} (error);
        \draw[-stealth] (x) -- node[midway,left] {} (error);
        \draw[-stealth] (y) -- node[midway,left] {} (error);
        %\draw[-stealth] (f) -- node[midway,left] {} (error);
        \draw[-stealth] (alpha) -- node[midway,left] {} (metatheta);
        \draw[-stealth] (alpha) -- node[midway,left] {} (theta);
        \draw[-stealth] (metatheta) -- node[midway,left] {} (metaS);
        \draw[-stealth] (metatau) -- node[midway,left] {} (error);
        \draw[-stealth] (metatheta) -- node[midway,left] {} (metaA);
        \draw[-stealth] (metaA) -- node[midway,left] {} (metatau);
        \draw[-stealth] (metaS) -- node[midway,left] {} (metatau);
        

      \end{tikzpicture}
      }
      \caption{Meta PAC guarantee (ours)}
      \label{fig:graph:ours}
    \end{subfigure}
    \caption{
        Comparison among different guarantees on prediction sets.
        {\color{red}An edge $A\to B$ between random variables $A,B$ represents that $B$ is drawn conditionally on $A$, and a plate with the symbol $N$ represents that there are $N$ copies of the variables in it, indexed by $i=1,\ldots,N$.}
        Each stripe pattern with a different color indicates that the corresponding random variables are {\color{red}simultaneously} conditioned on in the correctness guarantee;
        $F'$ denotes a conformal prediction set.
        {\color{red}Thus, for instance, in (d), there is a $1-\ep$ probability of correctness with respect to the test datapoint $(x,y)$, a $1-\alpha$ probability of correctness with respect to the test task and its adaptation data $(\theta,A)$, and a $1-\delta$ probability of correctness with respect to the calibration tasks, their calibration data, and their adaptation data $(\theta_i,S_i,A_i)$ for $i=1,\ldots,N$.}
        The proposed meta PAC prediction set (\ref{fig:graph:ours}) has the most fine-grained control over the correctness guarantee conditioning over calibration tasks, the test task and adaptation set, and the test data. 
    }
    \label{fig:setupdifference}
\end{figure}

We describe the problem on 
PAC prediction set construction for meta learning with adaptation; 
see Appendix \ref{apdx:prob:noadapt} for a simpler problem setup without adaptation, a special case of our main problem.

\textbf{Setup.} In the setting of Section \ref{ml}, the training samples from some training distributions $p_{\theta_i'}$, $i=1,\ldots,\nTraDS$ are used to learn a score function
via an \emph{arbitrary} meta learning method, {\color{red}including metric-based meta-learning \citep{snell2017prototypical} and optimization-based meta-learning \citep{finn2017model}}.
We denote the given meta-learned score function by $f$.
% calibration distributions
Additionally, we have
$\nCalDS$ calibration distributions $p_{\theta_1}, \dots, p_{\theta_\nCalDS}$, where
$\theta_1, \dots, \theta_\nCalDS$ is an i.i.d. sample from $p_\pi$.
From each calibration distribution $p_{\theta_i}$,
we draw $\nCalSam$ i.i.d. labeled examples for a calibration set,
\ie $(S_1, \dots, S_\nCalDS) \sim p_{\theta_1}^{\nCalSam} \cdots p_{\theta_\nCalDS}^{\nCalSam}$.
Additionally, we draw $t$ i.i.d. labeled examples for an adaptation set,
\ie $(A_1, \dots, A_\nCalDS) \sim p_{\theta_1}^{\nAdaSam} \cdots p_{\theta_\nCalDS}^{\nAdaSam}$;
we use them to construct the meta PAC prediction set.
% test distributions
Finally,
we consider a test distribution $p_{\theta}$, where
$\theta \sim p_\pi$. 
From it, we draw 
i.i.d. labeled adaptation examples $A$ and i.i.d. evaluation examples.

%{\color{red}
%goal
\textbf{Problem.} Our goal is to find a prediction set $F_\tau: \Zs^\nAdaSam \times \Xs \to 2^\Ys$ parametrized by $\tau \in \realnum_{\ge 0}$
which
satisfies a meta-learning variant of the PAC definition.
% notations
In particular, 
consider an estimator $\hat\tau_{\epsilon, \alpha, \delta}: \mathcal{Z}^{\nCalSam \times \nCalDS} \times \mathcal{Z}^{\nAdaSam \times \nCalDS} \to \TS$ that estimates
$\tau$ for a prediction set,
given an \emph{augmented calibration set} $(S_1, \dots, S_\nCalDS, A_1, \dots, A_\nCalDS)$.
Let $T_\epsilon(\theta, A)$ be a set of all $\epsilon$-correct parameters $\tau$ with respect to $f$ adapted using a test adaptation set $A$. % (which we also denote as $f^A$)
We also consider $F_\tau^A(x, y) \coloneqq F_\tau(A, x, y)$.

% correct
We say that
a prediction set $F_\tau$ parametrized by $\tau$
is $\epsilon$-correct for $p_{\theta}$ for a fixed adaptation set $A$,
if
$\tau \in T_\epsilon(\theta, A)$. 
% ``probably'' via an adaptation set
Moreover, we want the prediction set $F_\tau$ where $\tau$ is estimated via $\hat\tau_{\epsilon, \alpha, \delta}$ 
to be correct on most test sets $A$ for adaptation and for most test tasks $\theta$.
Letting $S_{1:k} \coloneqq (S_1, \dots, S_{k})$ and $A_{1:k} \coloneqq (A_1, \dots, A_{k})$ for any $k\ge 1$,
we want that, given 
$S_{1:\nCalDS} \in \mathcal{Z}^{\nCalSam \times \nCalDS}$
and
$A_{1:\nCalDS} \in \mathcal{Z}^{\nAdaSam \times \nCalDS}$,
\begin{align*}
  \Prob_{\theta, A} \[
  \hat\tau_{\epsilon, \alpha, \delta}(S_{1:\nCalDS}, A_{1:\nCalDS}) \in T_\epsilon(\theta, A)
  \] \ge 1 - \alpha,
\end{align*}
where 
$\theta \sim p_\pi$ and
$A \sim p_{\theta}^{\nAdaSam}$.
Intuitively, we want a prediction set, adapted via $A$, to be correct
on future labeled examples from $p_{\theta}$.
Finally, we want the above to hold for most augmented calibration sets $(S_{1:\nCalDS}, A_{1:\nCalDS})$ from most calibration tasks $\theta_1, \dots, \theta_{\nCalDS} \sim p_\pi$, leading to the following definition.

\footnotetext{It is also called a training-set conditional guarantee in \citep{vovk2013conditional}.}





% {\color{blue}
% %goal
% \textbf{Problem.} Our goal is to find a prediction set $f_\tau: \Zs^\nAdaSam \times \Xs \to 2^\Ys$ parametrized by an estimator
% $\hat\tau_{\epsilon, \alpha, \delta}: \mathcal{Z}^{\nCalSam \times \nCalDS} \times \mathcal{Z}^{\nAdaSam \times \nCalDS} \to \TS$,
% which
% satisfies a meta-learning variant of the PAC definition,
% given an augmented calibration set $(S_1, \dots, S_\nCalDS, A_1, \dots, A_\nCalDS)$ and a test adaptation set $A$.
% % correct
% In particular,
% recall that a prediction set $f_\tau$ parametrized by $\tau$
% is $\epsilon$-correct for $p_{\theta}$ if
% $\tau \in T_\epsilon(\theta, A)$,
% where $T_\epsilon(\theta, A)$ is a set of all $\epsilon$-correct parameters $\tau$ with respect to $f$ adapted using $A$.
% %(\ie $f_A$).


% % ``probably'' via an adaptation set
% We want the prediction set $f_{\hat\tau_{\epsilon, \alpha, \delta}}$ parametrized by the estimator $\hat\tau_{\epsilon, \alpha, \delta}$ 
% to be correct on most test sets for adaptation.
% Letting $S_{1:k} \coloneqq (S_1, \dots, S_{k})$ and $A_{1:k} \coloneqq (A_1, \dots, A_{k})$ for any $k\ge 1$,
% we want that, given 
% $S_{1:\nCalDS} \in \mathcal{Z}^{\nCalSam \times \nCalDS}$
% and
% $A_{1:\nCalDS} \in \mathcal{Z}^{\nAdaSam \times \nCalDS}$,
% \begin{align*}
%   \Prob_{\theta, A}[
%   \hat\tau_{\epsilon, \alpha, \delta}(S_{1:\nCalDS}, A_{1:\nCalDS}) \notin T_\epsilon(\theta, A)
%   ] \le \alpha,
% \end{align*}
% where 
% $\theta \sim p_\pi$ and
% $A \sim p_{\theta}^{\nAdaSam}$.
% Intuitively, we want a prediction set, adapted via $A$, to be correct
% on future labeled examples from $p_{\theta}$.
% Finally, we want the above to hold for most augmented calibration sets $(S_{1:\nCalDS}, A_{1:\nCalDS})$, leading to the following definition.
% }
\begin{definition}
  \label{def:mpac}
  An estimator $\hat{\tau}_{\epsilon,\alpha, \delta}: \Zs^{\nCalSam \times \nCalDS} \times \Zs^{\nAdaSam \times \nCalDS} \to \TS$ is \emph{$(\epsilon,\alpha,\delta)$-meta probably approximately correct (mPAC)} for $p_\pi$ if
\begin{align*}
  %\Probop_{\pi,p_{\theta_1}^{n_1},\dots,p_{\theta_\nCalDS}^{n_\nCalDS}} \! \left[
  \Prob_{\theta_{1:\nCalDS}, S_{1:\nCalDS}, A_{1:\nCalDS}} 
  \Bigg[
    %\Probop_{\pi, p_{\theta_{N+1}}^{n_{N+1}}}[
    \Prob_{\theta, A}  
    \Big[
        \hat{\tau}_{\epsilon,\alpha,\delta}(S_{1:\nCalDS}, A_{1:\nCalDS}) \in  T_{\epsilon}(\theta, A)
    \Big] \ge 1- \alpha
  \Bigg] \ge 1-\delta,
\end{align*}
where
$\theta_i, \theta \sim p_\pi$,
$S_i \sim p_{\theta_i}^{\nCalSam}$ for $i=1,\ldots,N$,
$S \sim p_{\theta}^{\nCalSam}$,
$A_i \sim p_{\theta_i}^{\nAdaSam}$ for $i=1,\ldots,N$,
and
$A \sim p_{\theta}^{\nAdaSam}$.
\end{definition}


% difference
Notably, Definition \ref{def:mpac} is tightly related to the PAC definition of meta conformal prediction \citep{fisch2021fewshot}.
We illustrate the difference in Figure \ref{fig:setupdifference};
the figure represents the different guarantees of prediction sets via graphical models. 
Each stripe pattern indicates the random variables that are conditioned on in the respective guarantee. 
Figure \ref{fig:graph:ours} represents the proposed guarantee, having Figure \ref{fig:graph:b} and \ref{fig:graph:d} as special cases. 
Figure \ref{fig:graph:meta-cp} shows the guarantee of meta conformal prediction proposed in \citep{fisch2021fewshot}, also having Figure \ref{fig:graph:a} and \ref{fig:graph:c} as special cases.
%
Figure \ref{fig:graph:ours} shows that the proposed correctness guarantee is conditioned over \emph{calibration tasks}, an \emph{adaptation set $A$ from a test task}, and \emph{test data $(x, y)$}. 
This implies that the correctness guarantee of an adapted prediction set (thus conditioned on the adaptation set) holds on most future test datasets from the same test task. 
In contrast, the guarantee in Figure \ref{fig:graph:meta-cp} is conditioned on the entire test task.
Thus, the correctness guarantee does not hold conditionally over adaptation sets; this means that the adapted prediction set (thus conditioned on an adaptation set) does not need to be correct over most future datasets in the same task. 

%\vspace{-2mm}
\subsection{Algorithm}

%% algorithm
\begin{algorithm}[th!]
  \caption{\textbf{Meta-PS}: PAC prediction set for meta-learning. Internally, any PAC prediction set algorithms are used to implement an estimator $\hat\tau_{\epsilon, \delta}$; 
  we use \textsc{PS-Binom} (Algorithm \ref{alg:cp}) in Appendix \ref{apdx:pacpsalg}.}
  \label{alg:meta_pac_ps}
  \small
  \begin{algorithmic}[1]  
    \Procedure{Meta-PS}{$S_{1:\nCalDS}$, $A_{1:\nCalDS}$, $f$, $g$, $\epsilon$, $\alpha$, $\delta$}
    \For{$i \in \{1, \dots, N\}$}
    \State $\hat{\tau}_{i} \gets \textsc{PS-Binom}(S_i, f^{A_i}, \epsilon, \alpha/2)$ \label{alg:taueforeachtask}
    %$\Comment{\text{$(\epsilon, \alpha/2)$-PAC prediction set from $S_i$}}$ 
    $\Comment{\text{Use Algorithm \ref{alg:cp} in Appendix \ref{apdx:pacpsalg}}}$
    \EndFor
    \State $S' \gets ((\hat{\tau}_{1}, 1), \dots, (\hat{\tau}_{\nCalDS}, 1))$ 
    \State $\hat\tau \gets \textsc{PS-Binom}(S', g, \alpha/2, \delta)$ \label{alg:finaltau}
    %$\Comment{\text{$(\alpha/2, \delta)$-PAC prediction set from $S'$}}$ 
    \State \textbf{return} $\hat\tau$ 
    \EndProcedure
    % \Procedure{PS}{$S$, $f$, $\epsilon$, $\delta$}
    % $\Comment{\text{Any algorithm for a given estimator $\hat\tau_{\epsilon, \delta}$.}}$
    % %\State \textbf{return} $\hat\tau_{\epsilon, \delta}(S)$ 
    
    % %$\Comment{\text{$\hat\tau_{\epsilon, \delta}$ implicitly depends on $f$}}$
    % \State \textbf{return} PS-Binom($S, f, \ep, \delta$)
    % \EndProcedure
  \end{algorithmic}
  %\vspace{-5mm}
\end{algorithm}


% algorithm
Next, we propose our meta PAC prediction set algorithm for an estimator $\hat{\tau}_{\epsilon,\alpha, \delta}$ that satisfies
Definition~\ref{def:mpac} while aiming to minimize the prediction set size,
% summary
by leveraging the scalar parameterization of a prediction set.
% details
The algorithm consists of two steps:
find a prediction set parameter over labeled examples $S_i$ and $A_i$ from the $i$-th calibration task distribution, and
find a prediction set over the parameter of prediction sets in the previous step.
At inference, 
the constructed prediction set is adapted to a test task distribution via an adaptation set $A$.
Importantly, in finding prediction sets (\ie implementating an $(\epsilon, \delta)$-PAC estimator $\hat\tau_{\epsilon, \delta}$), we can use any PAC prediction set algorithms (\eg Algorithm \ref{alg:cp} in Appendix \ref{apdx:pacpsalg}).


\textbf{Meta calibration.} 
% step 1
For the first step, for each $i\in \{1,\ldots, N\}$,
we estimate a prediction set parameter $\hat\tau_{\epsilon, \alpha/2}(S_i)$, satisfying a ($\epsilon$, $\alpha/2$)-PAC property
using a calibration set $S_i$ and a score function $f$ adapted via an adaptation set $A_i$, leading to $f^{A_i}$, by using any meta learning and adaptation algorithm.
We consider the $N$ learned prediction set parameters---with a dummy label $1$ to fit the convention of the PAC prediction set algorithm---to form a new labeled sample, \ie
$S' \coloneqq ((\hat{\tau}_{\epsilon,\alpha/2}(S_1), 1), \dots, (\hat{\tau}_{\epsilon,\alpha/2}(S_\nCalDS), 1))$.

% step 2
In the second part,
we construct an ($\alpha/2$, $\delta$)-PAC prediction set for the threshold $\tau$ using $S'$ and a score function $g$ defined as
$g(\tau, y) \coloneqq \tau \mathbbm{1}(y=1)$, where $\mathbbm{1}(\cdot)$ is the indicator function
\footnote{{\color{red}The constructed prediction set parameter is equivalent to $\tau$ satisfying $\Prob_S \[ \tau \le \hat\tau_{\epsilon, \alpha/2}(S) \] \ge 1 - \alpha/2$ with probability at least $1 - \delta$ over the randomness of $S_1, \dots, S_N$ used to estimate $\tau$.}}.
Thus, the constructed prediction set can be equivalently viewed as 
an interval $[\hat\tau_{\alpha/2, \delta}(S'),\infty)$ where
the thresholds $\tau$ of most calibration  distributions are included; see Section \ref{sec:theory} for a formal statement along with intuition on our design choice, and see Algorithm \ref{alg:meta_pac_ps} for an implementation.

%thus, having $\hat\tau_{\alpha/2, \delta}$ as the final prediction set parameter (\ie having $f_{\hat\tau_{\alpha/2, \delta}}$ as our meta prediction set) is a reasonable choice for satisfying the meta PAC guarantee in Definition \ref{def:mpac}; see Section \ref{sec:theory} for a formal statement and Algorithm \ref{alg:meta_pac_ps} for an implementation.

% The result can be viewed as a prediction set $[\hat\tau_{\alpha/2, \delta},\infty)$
% for $g$, 
% for future draws from the distribution. 
% Since $g=\tau$ over the distribution we consider, 
%  we propose 
% $f_{\hat\tau_{\alpha/2, \delta}}$ as the meta prediction set, defining the output threshold $\hat\tau_{\epsilon, \alpha, \delta}(S_{1:\nCalDS}, A_{1:\nCalDS})=\hat\tau_{\alpha/2, \delta}$.
% %the result of the second part is a threshold $\hat\tau'_{\alpha/2, \delta}$, such that $[\hat\tau_{\alpha/2, \delta},\infty) = g_{\hat\tau'_{\alpha/2, \delta}}$. 


% % intuition
% Intuitively,
% we have a sample of PAC thresholds learned on the calibration distributions. 
% Thus, the second step estimates a conservative choice for the parameter of the meta prediction set over the unknown test distribution. 


\textbf{Adaptation and inference.}
We then use labeled examples $A$ from a test distribution
to adapt the meta-learned score function $f$ as in the meta calibration part.
Then, we use the same parameter $\hat\tau_{\epsilon, \alpha, \delta}(S_{1:\nCalDS}, A_{1:\nCalDS})$ of the meta prediction set along with the adapted score function as our final meta prediction set $f_{\hat\tau_{\epsilon, \alpha, \delta}(S_{1:\nCalDS}, A_{1:\nCalDS})}$ for inference in the future. 

Reusing the same meta prediction set parameter after adaptation is valid, as the meta prediction set parameter is also chosen after adaptation via a hold-out adaptation set from the same distribution as each respective calibration set. Moreover, by reusing the same parameter, we only need a few labeled examples from the test distribution for an adaptation set, without requiring additional labeled examples for calibration on the test distribution.
Finally,  we rely on a PAC prediction set algorithm that aims  to minimize the expected prediction set size \citep{vovk2013conditional,Park2020PAC}; Algorithm \ref{alg:meta_pac_ps} relies on this property, thus making the meta prediction set size small. 

\vspace{-2mm}
\subsection{Theory}\label{sec:theory}
\vspace{-2mm}

The proposed Algorithm \ref{alg:meta_pac_ps} outputs a threshold for a prediction set that satisfies the mPAC guarantee, as stated in the following result (see Appendix \ref{apdx:thm:mpac_proof} for a proof):
\begin{theorem}\label{thm:mpac}
The estimator $\hat{\tau}_{\epsilon,\alpha,\delta}$ implemented in Algorithm \ref{alg:meta_pac_ps} is $(\epsilon,\alpha,\delta)$-mPAC for $p_\pi$.
\end{theorem}

% proof sketch
Intuitively, the algorithm implicitly constructs an interval $[\hat\tau_{\alpha/2, \delta}(S'),\infty)$ over scalar parameters of prediction sets. 
In particular, for the $i$-th distribution, the Algorithm in Line \ref{alg:taueforeachtask} finds a scalar parameter of a prediction set for the $i$-th distribution, which forms an empirical distribution over the scalar parameters. 
Due to the i.i.d. nature of $\theta_i$, $i=1,\ldots,N$, 
the parameter of a prediction set for a test distribution follows 
the same distribution over  scalar parameters. 
Thus, choosing a conservative scalar parameter as in Line \ref{alg:finaltau} of the  Algorithm suffices to satisfy the mPAC guarantee. 


% a prediction interval over scalar parameters of prediction sets. 
% In particular, for the $i$-th distribution, Algorithm Line \ref{alg:taueforeachtask} finds a scalar parameters of a prediction set for the $i$-th distribution, which forms an empirical distribution over the scalar parameters. 
% Due to the i.i.d. parameters $\theta_i$, 
% the parameter of a prediction set for a test distribution follows 
% the same distribution over the scalar parameters. 
% Thus, choosing a conservative scalar parameter as in Algorithm Line \ref{alg:finaltau} suffices to satisfy the mPAC guarantee. 

% \subsection{Applications}

% The proposed meta PAC prediction set is generally applicable to
% zero-shot learning and few-shot learning.
% Here, we mainly explain the application to few-shot learning,
% considering zero-shot learning as a special case of few-shot learning.

% \textbf{Few-shot learning.}
% The goal of few-shot learning is to adapt a score function and prediction set to
% a new distribution given only a few labeled examples.
% In this setup, we use a few labeled examples to adapt the underlying score function to
% the new distribution, while using the calibrated meta prediction set as it is.
% For zero-shot learning, we consider the same procedure without labeled examples.
% \SP{this section is not quite precise.}

% \textbf{Zero-shot learning.}


% %% In zero-shot learning \citep{TODO},
% %% the goal is to learn a score function and calibrate a meta prediction set
% %% such that the entire meta prediction set provides a PAC guarantee of a new distribution.
% %% Our method is applicable to zero-shot learning by simply without considering adaptation samples.
% %% \SP{should we add this without empirical justification?}


% %% \textbf{Unsupervised domain adaptation.}
% %% The goal of unsupervised domain adaptation \citep{TODO} is to
% %% learn a score function and calibrate a prediction set
% %% by leveraging unlabeled examples from a new distribution.
% %% Our method is also applicable to the unsupervised domain adaptation by
% %% updating a score function using unlabeled examples
% %% via known unsupervised domain adaptation methods.
% %% \SP{should we add this without empirical justification?}





==> utils/header.tex <==


\usepackage{amsmath} 
\usepackage{bbm} % for mathbbm
\usepackage{amsthm}
\usepackage{amsfonts}

\makeatletter
\@ifundefined{proposition}{%
    \newtheorem{proposition}{Proposition}
}{}
\@ifundefined{definition}{%
    \newtheorem{definition}{Definition}%
}{}
\@ifundefined{lemma}{%
    \newtheorem{lemma}{Lemma}
}{}
\@ifundefined{corollary}{%
    \newtheorem{corollary}{Corollary}
}{}
\@ifundefined{theorem}{%
    \newtheorem{theorem}{Theorem}
}{}
\@ifundefined{corollary}{%
    \newtheorem{corollary}{Corollary}
}{}
\@ifundefined{assumption}{%
    \newtheorem{assumption}{Assumption}
}{}
\@ifundefined{problem}{%
    \newtheorem{problem}{Problem}
}{}
\@ifundefined{problem*}{%
    \newtheorem*{problem*}{Problem}
}{}
\@ifundefined{claim}{%
    \newtheorem{claim}{claim}
}{}

\theoremstyle{remark}
\@ifundefined{example}{%
    \newtheorem{example}{Example}
}{}

\makeatother




%% shorthands for labels, equations, matrices...
\providecommand{\eqnref}			[1]		{Equation~(\ref{#1})}
\providecommand{\tabref}			[1]		{Table~\ref{#1}}
\providecommand{\figref}			[1]		{Figure~\ref{#1}}
\providecommand{\alref}			[1]		{Algorithm~\ref{#1}}
\providecommand{\defref}			[1]		{Definition~\ref{#1}}
\providecommand{\prbref}			[1]		{Problem~\ref{#1}}
\providecommand{\thmref}			[1]		{Theorem~\ref{#1}}
\providecommand{\proref}			[1]		{Proposition~\ref{#1}}
\providecommand{\lemref}			[1]		{Lemma~\ref{#1}}
\providecommand{\corref}			[1]		{Corollary~\ref{#1}}
\providecommand{\secref}			[1]		{Section~\ref{#1}}
\providecommand{\apxref}			[1]		{Appendix~\ref{#1}}

\providecommand{\eqa}				[1]		{\begin{align}#1\end{align}}
\providecommand{\eqas}			[1]		{\begin{align*}#1\end{align*}}
\providecommand{\eqml}			[1]		{\begin{multline}#1\end{multline}}
\providecommand{\mat}				[2]		{\left[\begin{array}{#1} #2 \end{array}\right]}

%% shorthands for abbreviations for Latin terms.
\providecommand{\ie}{\emph{i.e.,}~}
\providecommand{\eg}{\emph{e.g.,}~}


%% Number types
\providecommand{\realnum}					{\mathbb{R}}
\providecommand{\integernum}				{\mathbb{Z}}
\providecommand{\complexnum}				{\mathbb{C}}
\providecommand{\naturalnum}				{\mathbb{N}}

%% Common mathematical functions and symbols
\renewcommand{\(}						{\left(}
\renewcommand{\)}						{\right)}
\renewcommand{\[}						{\left[}
\renewcommand{\]}						{\right]}
\newcommand{\<}						{\left<}
\renewcommand{\>}						{\right>}

%% shorthands for useful functions, expectation, probability, indicator function
\providecommand{\Prob}{\mathbbm{P}}
\providecommand{\Probop}{\mathop{\Prob}}
\providecommand{\Exp}{\mathbbm{E}}
\providecommand{\Expop}{\mathop{\Exp}}
\providecommand{\Ind}{\mathbbm{I}}
\providecommand{\iid}{i.i.d.}
\providecommand{\findop}{\mathop{\text{find}}}

% hat
\def\ah{\hat{{a}}}
\def\bh{\hat{{b}}}
\def\ch{\hat{{c}}}
\def\dh{\hat{{d}}}
\def\eh{\hat{{e}}}
\def\fh{\hat{{f}}}
\def\gh{\hat{{g}}}
\def\hh{\hat{{h}}}
\def\ih{\hat{{i}}}
\def\ih{\hat{{j}}}
\def\kh{\hat{{k}}}
\def\lh{\hat{{l}}}
\def\mh{\hat{{m}}}
\def\nh{\hat{{n}}}
\def\oh{\hat{{o}}}
\def\ph{\hat{{p}}}
\def\qh{\hat{{q}}}
\def\rh{\hat{{r}}}
\def\sh{\hat{{s}}}
\def\th{\hat{{t}}}
\def\uh{\hat{{u}}}
\def\vh{\hat{{v}}}
\def\wh{\hat{{w}}}
\def\xh{\hat{{x}}}
\def\yh{\hat{{y}}}
\def\zh{\hat{{z}}}
\def\Ah{\hat{{A}}}
\def\Bh{\hat{{B}}}
\def\Ch{\hat{{C}}}
\def\Dh{\hat{{D}}}
\def\Eh{\hat{{E}}}
\def\Fh{\hat{{F}}}
\def\Gh{\hat{{G}}}
\def\Hh{\hat{{H}}}
\def\Ih{\hat{{I}}}
\def\Jh{\hat{{J}}}
\def\Kh{\hat{{K}}}
\def\Lh{\hat{{L}}}
\def\Mh{\hat{{M}}}
\def\Nh{\hat{{N}}}
\def\Oh{\hat{{O}}}
\def\Ph{\hat{{P}}}
\def\Qh{\hat{{Q}}}
\def\Rh{\hat{{R}}}
\def\Sh{\hat{{S}}}
\def\Th{\hat{{T}}}
\def\Uh{\hat{{U}}}
\def\Vh{\hat{{V}}}
\def\Wh{\hat{{W}}}
\def\Xh{\hat{{X}}}
\def\Yh{\hat{{Y}}}
\def\Zh{\hat{{Z}}}
%% hat of greek letters
\def\rhoh{\hat{\rho}}
\def\pih{\hat{\pi}}
\def\tauh{\hat{\tau}}

%
%% bar
%\def\ab{\bar{{a}}}
%\def\bb{\bar{{b}}}
%\def\cb{\bar{{c}}}
\def\db{\bar{{d}}}
%\def\eb{\bar{{e}}}
%\def\fb{\bar{{f}}}
%\def\gb{\bar{{g}}}
%\def\hb{\bar{{h}}}
%\def\ib{\bar{{i}}}
%\def\ib{\bar{{j}}}
%\def\kb{\bar{{k}}}
%\def\lb{\bar{{l}}}
%\def\mb{\bar{{m}}}
%\def\nb{\bar{{n}}}
%\def\ob{\bar{{o}}}
%\def\pb{\bar{{p}}}
%\def\qb{\bar{{q}}}
%\def\rb{\bar{{r}}}
%\def\sb{\bar{{s}}}
%\def\tb{\bar{{t}}}
%\def\ub{\bar{{u}}}
%\def\vb{\bar{{v}}}
%\def\wb{\bar{{w}}}
%\def\xb{\bar{{x}}}
\def\yb{\bar{{y}}}
%\def\zb{\bar{{z}}}
%\def\Ab{\bar{{A}}}
%\def\Bb{\bar{{B}}}
%\def\Cb{\bar{{C}}}
%\def\Db{\bar{{D}}}
%\def\Eb{\bar{{E}}}
%\def\Fb{\bar{{F}}}
%\def\Gb{\bar{{G}}}
%\def\Hb{\bar{{H}}}
%\def\Ib{\bar{{I}}}
%\def\Jb{\bar{{J}}}
%\def\Kb{\bar{{K}}}
%\def\Lb{\bar{{L}}}
%\def\Mb{\bar{{M}}}
%\def\Nb{\bar{{N}}}
%\def\Ob{\bar{{O}}}
%\def\Pb{\bar{{P}}}
%\def\Qb{\bar{{Q}}}
%\def\Rb{\bar{{R}}}
%\def\Sb{\bar{{S}}}
%\def\Tb{\bar{{T}}}
%\def\Ub{\bar{{U}}}
%\def\Vb{\bar{{V}}}
%\def\Wb{\bar{{W}}}
%\def\Xb{\bar{{X}}}
%\def\Yb{\bar{{Y}}}
%\def\Zb{\bar{{Z}}}
%

%% script 
\def\as{\mathcal{{a}}}
\def\bs{\mathcal{{b}}}
\def\cs{\mathcal{{c}}}
\def\ds{\mathcal{{d}}}
\def\es{\mathcal{{e}}}
\def\fs{\mathcal{{f}}}
\def\gs{\mathcal{{g}}}
\def\hs{\mathcal{{h}}}
\def\is{\mathcal{{i}}}
\def\is{\mathcal{{j}}}
\def\ks{\mathcal{{k}}}
\def\ls{\mathcal{{l}}}
\def\ms{\mathcal{{m}}}
\def\ns{\mathcal{{n}}}
\def\os{\mathcal{{o}}}
\def\ps{\mathcal{{p}}}
\def\qs{\mathcal{{q}}}
\def\rs{\mathcal{{r}}}
\def\ss{\mathcal{{s}}}
\def\ts{\mathcal{{t}}}
\def\us{\mathcal{{u}}}
\def\vs{\mathcal{{v}}}
\def\ws{\mathcal{{w}}}
\def\xs{\mathcal{{x}}}
\def\ys{\mathcal{{y}}}
\def\zs{\mathcal{{z}}}
\def\As{\mathcal{{A}}}
\def\Bs{\mathcal{{B}}}
\def\Cs{\mathcal{{C}}}
\def\Ds{\mathcal{{D}}}
\def\Dsh{\hat{\mathcal{{D}}}}
\def\Es{\mathcal{{E}}}
\def\Fs{\mathcal{{F}}}
\def\Gs{\mathcal{{G}}}
\def\Gsh{\hat{\mathcal{{G}}}}
\def\Hs{\mathcal{{H}}}
\def\Hsh{\hat{\mathcal{{H}}}}
\def\Is{\mathcal{{I}}}
\def\Js{\mathcal{{J}}}
\def\Ks{\mathcal{{K}}}
\def\Ksh{\hat{\mathcal{{K}}}}
\def\Ksb{\bar{\mathcal{{K}}}}
\def\Ls{\mathcal{{L}}}
\def\Ms{\mathcal{{M}}}
\def\Ns{\mathcal{{N}}}
\def\Os{\mathcal{{O}}}
\def\Ps{\mathcal{{P}}}
\def\Qs{\mathcal{{Q}}}
\def\Rs{\mathcal{{R}}}
\def\Ss{\mathcal{{S}}}
\def\Ts{\mathcal{{T}}}
\def\Us{\mathcal{{U}}}
\def\Vs{\mathcal{{V}}}
\def\Ws{\mathcal{{W}}}
\def\Xs{\mathcal{{X}}}
\def\Ys{\mathcal{{Y}}}
\def\Zs{\mathcal{{Z}}}
%



